Leveraging Expert Guided Adversarial Augmentation For Improving Generalization in Named Entity Recognition

Named Entity Recognition (NER) systems often demonstrate great performance on in-distribution data, but perform poorly on examples drawn from a shifted distribution. One way to evaluate the generalization ability of NER models is to use adversarial examples, on which the specific variations associated with named entities are rarely considered. To this end, we propose leveraging expert-guided heuristics to change the entity tokens and their surrounding contexts thereby altering their entity types as adversarial attacks. Using expert-guided heuristics, we augmented the CoNLL 2003 test set and manually annotated it to construct a high-quality challenging set. We found that state-of-the-art NER systems trained on CoNLL 2003 training data drop performance dramatically on our challenging set. By training on adversarial augmented training examples and using mixup for regularization, we were able to significantly improve the performance on the challenging set as well as improve out-of-domain generalization which we evaluated by using OntoNotes data. We have publicly released our dataset and code at https://github.com/GT-SALT/Guided-Adversarial-Augmentation.

==> Most_updated_table_11_12.tex <==

\begin{table*}[ht]
\centering
% \begin{tabular}{p{0.1\linewidth} | p{0.22\linewidth} | p{0.18\linewidth} | p{0.21\linewidth} | p{0.16\linewidth}}
\begin{tabular}{c!{\vrule width 2pt}c!{\vrule width 2pt}c|c|c!{\vrule width 2pt}c|c|c}
\hline\cline{1-8}
\multicolumn{2}{c|}{}&
\multicolumn{3}{c|}{\textbf{0-Shot}}&
\multicolumn{3}{c|}{\textbf{5-Shot}}\\
\hline
\textbf{Percent} & \textbf{Model} & \textbf{ID} & \textbf{CS}& \textbf{OOD}& \textbf{ID} & \textbf{CS}  & \textbf{OOD}\\
\hline\cline{1-8}
\textbf{N/A} & \multirow{BERT} &          90.82 &    71.80     &   59.07      &      90.75 & 72.66 &58.72\\ 
\hline\cline{1-8}
\textbf{N/A} & \multirow{BERT + TAVAT} &   91.82  &   70.14    &   0.3322      &  91.38&  74.36   &0.3295\\ 
\hline\cline{1-8}
\textbf{5\%} & \multirow{BERT + AT} &  89.48 & 80.39  & 60.34 &      90.91&      84.47       &  59.23\\ 
\cline{2-8}
& \multirow{BERT + AT + Dropout} &        90.77 &      83.37   &    61.16     &  90.93&  83.74&  62.24 \\ 
\cline{2-8}
& \multirow{BERT + AT + Mixup} & \textbf{90.84} & \textbf{85.92} & 60.87 &  90.46& 82.79 & 61.54\\ 
\cline{2-8}
& \multirow{BERT + TextFlint} & 89.70 & 56.76 & 64.67 &  89.59& 52.99 & 67.46\\ 
\hline\cline{1-8}
\textbf{10\%} & \multirow{BERT + AT} & 90.37 & 86.16 &59.07  &  \textbf{91.18}& \textbf{85.83} &61.09 \\ 
\cline{2-8}
& \multirow{BERT + AT + Dropout} & 90.1 & 84.97& 62.5 &   90.87& 84.19 & 61.86 \\ 
\cline{2-8}
& \multirow{BERT + AT + Mixup} & \textbf{90.79} & \textbf{88.79} & 58.33 &  89.55& 84.66 & \textbf{67.47}
 \\
\cline{2-8}
& \multirow{BERT + TextFlint} & 88.85 &54.04  &\textbf{69.05}  &  89.14&53.32  &66.67 \\
\hline\cline{1-8}
\textbf{30\%} & \multirow{BERT + AT} & 90.84 &86.42 & 56.65 & 90.72 & 85.42  &60.76\\
\cline{2-8}
& \multirow{BERT + AT + Dropout} & \textbf{90.93} & 86.91 &  62.24   & \textbf{90.75} &\textbf{87.97} &61.6 \\ 
\cline{2-8}
& \multirow{BERT + AT + Mixup} & 90.85 & \textbf{87.30} & 59.66 &  90.51& 81.23  &\textbf{69.46}\\ 
\cline{2-8}
& \multirow{BERT + TextFlint} & 89.71 & 60.32 & \textbf{64.29}  &  88.18&56.64 & 65.88\\
\hline\cline{1-8}
\textbf{50\%} & \multirow{BERT + AT} & 90.85 &87.50 & 59.17   &  \textbf{91.11}& \textbf{90.41}&62.18 \\ 
\cline{2-8}
& \multirow{BERT + AT + Dropout} & 90.19 & \textbf{88.88} & \textbf{63.29} &  90.2& 85.8 &60.83 \\ 
\cline{2-8}
& \multirow{BERT + AT + Mixup} &\textbf{90.92} & 88.00 & 60.09 & 89.64& 84.88 &\textbf{67.47} \\ 
\cline{2-8}
& \multirow{BERT + TextFlint} & 89.55 & 53.49 &62.72  &  89.05& 59.93 &65.48 \\
\hline\cline{1-8}
\textbf{100\%} & \multirow{BERT + AT} & 90.52 &  87.74  & 57.14 &  \textbf{90.82}& 90.34 &57.76 \\ 
\cline{2-8}
& \multirow{BERT + AT + Dropout} &90.16  & 88.45 & 61.28 &  90.76& 88.46 &60.25 \\ 
\cline{2-8}
& \multirow{BERT + AT + Mixup} & \textbf{90.53} & \textbf{90.21} &59.92 &   89.40& \textbf{91.33}  & 67.07\\ 
\cline{2-8}
& \multirow{BERT + TextFlint} &87.31  &59.12  &\textbf{63.47} &  85.83 & 60.43 & \textbf{69.05}\\
\hline
\end{tabular}
\caption{F1 Scores on the Original CoNLL 2003 Test Set (ID) and its Challenging Set (CS); Expert-Guided Augmented Data for Training (AT)}
\label{tab:f1_main_results}
\end{table*}

==> newest_table.tex <==

\begin{table*}[ht]
\centering
% \begin{tabular}{p{0.1\linewidth} | p{0.22\linewidth} | p{0.18\linewidth} | p{0.21\linewidth} | p{0.16\linewidth}}
\begin{tabular}{c!{\vrule width 2pt}c!{\vrule width 2pt}c|c|c!{\vrule width 2pt}c|c|c}
\hline
\multicolumn{2}{c|}{}&
\multicolumn{3}{c|}{\textbf{0-Shot}}&
\multicolumn{3}{c|}{\textbf{5-Shot}}\\
\hline
\textbf{Percent} & \textbf{Model} & \textbf{ID} & \textbf{CS}& \textbf{OOD}& \textbf{ID} & \textbf{CS}  & \textbf{OOD}\\
\hline\cline{1-8}
\textbf{N/A} & \multirow{BERT} &          90.82 &    71.80     &   59.07      &      90.75 & 72.66 &58.72\\ 
\hline\cline{1-8}
\textbf{N/A} & \multirow{BERT + TAVAT} &   91.82  &   70.14    &   0.3322      &  91.38&  74.36   &0.3295\\ 
\hline\cline{1-8}
\textbf{5\%} & \multirow{BERT + AT} &  89.48 & 80.39  & 60.34 &      90.91&      84.47       &  59.23\\ 
\cline{2-8}
& \multirow{BERT + AT + Dropout} &        90.77 &      83.37   &    61.16     &  90.93&  83.74&  62.24 \\ 
\cline{2-8}
& \multirow{BERT + AT + Mixup} & \textbf{90.84} & \textbf{85.92} & 60.87 &  90.46& 82.79 & 61.54\\ 
\cline{2-8}
& \multirow{BERT + TextFlint} & 89.70 & 56.76 & 64.67 &  89.59& 52.99 & 67.46\\ 
\hline\cline{1-8}
\textbf{10\%} & \multirow{BERT + AT} & 90.37 & 86.16 &59.07  &  91.18& 85.83 &61.09 \\ 
\cline{2-8}
& \multirow{BERT + AT + Dropout} & 90.1 & 84.97& 62.5 &   90.87& 84.19 & 61.86 \\ 
\cline{2-8}
& \multirow{BERT + AT + Mixup} & \textbf{90.79} & \textbf{88.79} & 58.33 &  90.85& 87.22 & 62.76 \\
\cline{2-8}
& \multirow{BERT + TextFlint} & 88.85 &54.04  &69.05  &  89.14&53.32  &66.67 \\
\hline\cline{1-8}
\textbf{30\%} & \multirow{BERT + AT} & 90.84 &86.42 & 56.65 & 90.72 & 85.42  &60.76\\
\cline{2-8}
& \multirow{BERT + AT + Dropout} & \textbf{90.93} & 86.91 &  \textbf{62.24}   & 90.75 &87.97 &61.6 \\ 
\cline{2-8}
& \multirow{BERT + AT + Mixup} & 90.85 & \textbf{87.30} & 59.66 &  90.87& 86.83  &62.5\\ 
\cline{2-8}
& \multirow{BERT + TextFlint} & 89.71 & 60.32 & 64.29  &  88.18&56.64 & 65.88\\
\hline\cline{1-8}
\textbf{50\%} & \multirow{BERT + AT} & 90.85 &87.50 & 59.17   &  91.11& 90.41&62.18 \\ 
\cline{2-8}
& \multirow{BERT + AT + Dropout} & 90.19 & \textbf{88.88} & \textbf{63.29} &  90.2& 85.8 &60.83 \\ 
\cline{2-8}
& \multirow{BERT + AT + Mixup} &\textbf{90.92} & 88.00 & 60.09 & 89.76& 88.32 &\textbf{63.86} \\ 
\cline{2-8}
& \multirow{BERT + TextFlint} & 89.55 & 53.49 &62.72  &  89.05& 59.93 &65.48 \\
\hline\cline{1-8}
\textbf{100\%} & \multirow{BERT + AT} & 90.52 &  87.74  & 57.14 &  90.82& 90.34 &57.76 \\ 
\cline{2-8}
& \multirow{BERT + AT + Dropout} &90.16  & 88.45 & \textbf{61.28} &  90.76& 88.46 &60.25 \\ 
\cline{2-8}
& \multirow{BERT + AT + Mixup} & \textbf{90.53} & \textbf{90.21} &59.92 &   90.81&86.59  & 60.43\\ 
\cline{2-8}
& \multirow{BERT + TextFlint} &87.31  &59.12  &63.47 &  85.83 & 60.43 & 69.05\\
\hline
\end{tabular}
\caption{F1 Scores on the Original CoNLL 2003 Test Set (ID) and its Challenging Set (CS); Expert-Guided Augmented Data for Training (AT)}
\label{tab:f1_main_results}
\end{table*}

==> old_introduction.tex <==
\section{Introduction}

Deep learning models have achieved great performance on many NLP problems \cite{devlin-etal-2019-bert, bahdanau2016neural}.  However they have been shown to rely on spurious correlations, which consist of prediction rules that may hold for the majority of examples but not in general \cite{DBLP:journals/corr/abs-2007-06778, kaushik-lipton-2018-much, poliak2018hypothesis, gururangan-etal-2018-annotation}. So while it has been demonstrated that while deep learning models may perform very well on the In Distribution, they often perform much worse on examples drawn from an Out-of-Distribution test set where these correlations may no longer be true. \cite{DBLP:journals/corr/abs-1904-01130, DBLP:journals/corr/abs-2007-06778, glockner2018breaking, mccoy2019right, nie2018analyzing}

There have been several works incorporating the construction of challenging/adversarial datasets for the purpose of bench-marking the state of the art models' performances on Out-of-Distribution examples. In \cite{kaushik2020learning}, their work involves the use of a human expert for counterfactually manipulating text in order to "disentangle the spurious and non-spurious associations" in the Natural Language Inference problem setting. In \cite{DBLP:journals/corr/abs-1904-01130}, they generate a challenging dataset from the Quora Question Pairs (QQP) dataset by utilizing controlling word swapping and backtranslations. In \cite{glockner2018breaking}, they generate an augmented NLI test set with examples incorporating different kinds of lexical knowledge.

So while many previous works have constructed challenging datasets for NLI, Named Entity Recognition (NER) as a key problem setting for deep learning systems involving the classification of the semantic categories of entities (e.g., organizations, locations)  \cite{jbp:/content/journals/10.1075/li.30.1.03nad} is in still need of improved benchmarks of true generalization.  This raises the question of what linguistic patterns govern some of the hard cases for present neural models in NER who's utilization for the generation of adversarial examples would provide the dataset for benchmarking generalization?

There are several other works that explore hard cases in NER. In \cite{fu2020rethinking}, they analyze the generalization of models using measures they propose. They propose a measure called consistency, and conclude that if two named entity label categories have low consistency then the model will often have difficulty distinguishing between them. They go on to define Overlapping Categories as a hard case that occurs when two named entity label categories have overlapping entities. In \cite{stanislawek-etal-2019-named}, they identify Sentence level context cases where the correct named entity label category can only be determined when the specific sentence context that contains it is taken into consideration. They identified General ambiguity cases as situations where an entity occurs in a different sense than the sense in which the word is most often used. They also define General hard cases as cases that occur in a set for the first time in a certain sub-type and can be interpreted in different ways. 


There are several works exploring specifically the generation of adversarial examples by applying changes directly to text for the NER problem setting. In \cite{gui2021textflint}, they define augmentations specifically for NER, however their's are less focused on the context than ours. Theirs involve concatenating sentences, swapping/inserting/deleting a random character in an entity, entity swapping with OOV entities, and CrossCategory which involves the swapping of an named entity with one that has a different label. Ours is different from their defined augmentation because theirs inserts a random entity of a different label, while ours only alters part of the named entity and/or the surrounding context to change the label.

In \cite{zeng-etal-2020-counterfactual}, they investigate spurious correlations from a causal perspective exploring the relationship between the entity and its surrounding context. They randomly select an entity to replace the selected entity with but only select entities of the same label to preserve linguistic correctness. We purposely alter the entity with the goal of changing the label to target the NER hard cases. They also make use of an example discriminator to ensure that the augmented example does not bring in noise and thus lower model performance. Through our use of Mixup, we allow for our model to be trained on the generated noise without causing a great degree of degraded performance.

The mixup data augmentation technique was proposed in \cite {zhang2018mixup}. It was demonstrated by training an image classifier on linear interpolations of randomly sampled image data. Given a pair of data points (x,y) and (x',y'), where x denotes an image in the raw pixel space, and y denotes the label in a one-hot representation. The mixup technique then creates a new data point by the interpolation of the images and their labels as shown in the following equations:
\begin{equation} \hat{x}= \lambda x +(1 - \lambda) \tilda{x}  \end{equation}
\begin{equation} \hat{y}= \lambda y +(1 - \lambda) \tilda{y}  \end{equation}

$\lambda$ is drawn from a Beta distribution. Mixup is training the neural network for image classification by the minimization of the loss on the virtual examples. The linear interpolation of the data points creates a virtual vicinity distribution around the original data space causing the improvement of the classifier's generalization performance when being trained on the interpolated data points. 

There has been work exploring Mixup's performance on Out-of-distribution data. \cite{thulasidasan2020mixup, verma2019manifold} show how using mixup allows neural models to be less confident during distribution shifts than models not using mixup. \cite{8478159} shows how mixup allows models to have a smoother decision-making surface than ERM allowing for more robustness to adversarial examples, and in \cite{pang2020mixup}, they developed an inference principle to allow for mixup models to better handle adversarial examples.


==> old_table.tex <==
\begin{table*}[ht]
\centering
% \begin{tabular}{p{0.1\linewidth} | p{0.22\linewidth} | p{0.18\linewidth} | p{0.21\linewidth} | p{0.16\linewidth}}
\begin{tabular}{c|l|c|c|c}
\hline
\textbf{Percent} & \textbf{Model} & \textbf{In Distribution} &  \textbf{Challenge Set}&  \textbf{Out-of-Domain} \\
\hline\cline{1-8}
\textbf{N/A} & \multirow{BERT} & 90.82 \hspace*{2 mm}\vert \hspace*{2 mm}  90.75 & 71.80 \hspace*{2 mm}\vert \hspace*{2 mm} 72.66  & 59.07  \hspace*{2 mm}\vert \hspace*{2 mm}  58.72\\ 
\hline\cline{1-8}
\textbf{N/A} & \multirow{BERT + TAVAT} &91.82  \hspace*{2 mm}\vert \hspace*{2 mm}  91.38 &70.14  \hspace*{2 mm}\vert \hspace*{2 mm} 74.36 & 0.3322 \hspace*{2 mm}\vert \hspace*{2 mm} 0.3295\\ 
\hline\cline{1-8}
\textbf{5\%} & \multirow{BERT + AT} & 89.48 \hspace*{2 mm}\vert \hspace*{2 mm} 90.91 & 80.39 \hspace*{2 mm}\vert \hspace*{2 mm} 84.47 & 60.34  \hspace*{2 mm}\vert \hspace*{2 mm} 59.23\\ 
\cline{2-5}
& \multirow{BERT + AT + Dropout} & 90.77 \hspace*{2 mm}\vert \hspace*{2 mm} 90.93 & 83.37 \hspace*{2 mm}\vert \hspace*{2 mm}  83.74 &61.16 \hspace*{2 mm}\vert \hspace*{2 mm} 62.24 \\ 
\cline{2-5}
& \multirow{BERT + AT + Mixup} & \textbf{90.84} \hspace*{2 mm}\vert \hspace*{2 mm}  90.46 & \textbf{85.92} \hspace*{2 mm}\vert \hspace*{2 mm}  82.79 & 60.87  \hspace*{2 mm}\vert \hspace*{2 mm} 61.54\\ 
\cline{2-5}
& \multirow{BERT + TextFlint} &     &      &   \\ 
\hline\cline{2-8}
\textbf{10\%} & \multirow{BERT + AT} & 90.37  91.18  &86.16   85.83  & 59.07  61.09 \\ 
\cline{2-5}
& \multirow{BERT + AT + Dropout} & 90.1  90.87 &84.97    84.19  & 62.5   61.86 \\ 
\cline{2-5}
& \multirow{BERT + AT + Mixup} & \textbf{90.79}   90.85 & \textbf{88.79}  87.22  & 58.33   62.76 \\
\cline{2-5}
& \multirow{BERT + TextFlint} &     &     &    \\
\hline\cline{2-8}
\textbf{30\%} & \multirow{BERT + AT} & 90.84  90.72  &86.42    85.42 & 56.65  60.76\\
\cline{2-5}
& \multirow{BERT + AT + Dropout} & \textbf{90.93}   90.75 &  86.91   87.97  & \textbf{62.24}  61.6 \\ 
\cline{2-5}
& \multirow{BERT + AT + Mixup} & 90.85   90.87 & \textbf{87.30}   86.83 &  59.66  62.5\\ 
\cline{2-5}
& \multirow{BERT + TextFlint} &     &     &    \\
\hline\cline{2-8}
\textbf{50\%} & \multirow{BERT + AT} & 90.85  91.11 & 87.50    90.41 & 59.17  62.18 \\ 
\cline{2-5}
& \multirow{BERT + AT + Dropout} & 90.19   90.2 & \textbf{88.88}   85.8 & \textbf{63.29}  60.83 \\ 
\cline{2-5}
& \multirow{BERT + AT + Mixup} &\textbf{90.92}   90.6 & 88.00  88.34 & 60.09  61.6 \\ 
\cline{2-5}
& \multirow{BERT + TextFlint} &     &     &    \\
\hline\cline{2-8}
\textbf{100\%} & \multirow{BERT + AT} & 90.52   90.82 &  87.74   90.34  & 57.14  57.76 \\ 
\cline{2-5}
& \multirow{BERT + AT + Dropout} &90.16    90.76 & 88.45   88.46 & \textbf{61.28}  60.25 \\ 
\cline{2-5}
& \multirow{BERT + AT + Mixup} & \textbf{90.53}  90.81  & \textbf{90.21}   86.59 & 59.92   60.43\\ 
\cline{2-5}
& \multirow{BERT + TextFlint} &     &     &    \\
\hline
\end{tabular}
\caption{F1 Scores on the Original CoNLL 2003 Test Set (ID) and its Challenging Set (CS); Expert-Guided Augmented Data for Training (AT); F1 Scores on the first 50 examples from the OntoNotes Out-of-Domain test set (OOD) that have a percentage of entity tokens out of all tokens that is greater than 49\%.}
\label{tab:f1_main_results}
\end{table*}

==> table2.tex <==
\begin{table*}[ht]
\centering
% \begin{tabular}{p{0.1\linewidth} | p{0.22\linewidth} | p{0.18\linewidth} | p{0.21\linewidth} | p{0.16\linewidth}}
\begin{tabular}{c|l|c|c|c|c|c|c}
\hline
\multicolumn{2}{c|}{}&
\multicolumn{3}{c|}{\textbf{0-Shot}}&
\multicolumn{3}{c|}{\textbf{5-Shot}}\\
\hline
\textbf{Percent} & \textbf{Model} & \textbf{ID} & \textbf{ID}& \textbf{CS}& \textbf{CS} & \textbf{OOD}  & \textbf{OOD}\\
\hline\cline{1-8}
\textbf{N/A} & \multirow{BERT} & 90.82 & 90.75 & 71.80 & 72.66  & 59.07 & 58.72\\ 
\hline\cline{1-8}
\textbf{N/A} & \multirow{BERT + TAVAT} &91.82  & 91.38 &70.14   & 74.36 & 0.3322  & 0.3295\\ 
\hline\cline{1-8}
\textbf{5\%} & \multirow{BERT + AT} & 89.48 & 90.91 & 80.39 & 84.47 & 60.34 &  59.23\\ 
\cline{2-8}
& \multirow{BERT + AT + Dropout} & 90.77 & 90.93 & 83.37 & 83.74 &61.16 &62.24 \\ 
\cline{2-8}
& \multirow{BERT + AT + Mixup} & \textbf{90.84} & 90.46 & \textbf{85.92} & 82.79 & 60.87 & 61.54\\ 
\cline{2-8}
& \multirow{BERT + TextFlint} & 89.70 & 89.59 &56.76  &52.99  &64.67  & 67.46\\ 
\hline\cline{1-8}
\textbf{10\%} & \multirow{BERT + AT} & 90.37 &91.18  &86.16  &85.83  & 59.07 &61.09 \\ 
\cline{2-8}
& \multirow{BERT + AT + Dropout} & 90.1 &90.87 &84.97  & 84.19  & 62.5 & 61.86 \\ 
\cline{2-8}
& \multirow{BERT + AT + Mixup} & \textbf{90.79} & 90.85 & \textbf{88.79} &87.22  & 58.33 & 62.76 \\
\cline{2-8}
& \multirow{BERT + TextFlint} & 88.85 & 89.14 & 54.04 & 53.32 & 69.05 &66.67 \\
\hline\cline{1-8}
\textbf{30\%} & \multirow{BERT + AT} & 90.84 &90.72  &86.42  & 85.42 & 56.65 &60.76\\
\cline{2-8}
& \multirow{BERT + AT + Dropout} & \textbf{90.93} & 90.75 &  86.91  &87.97  & \textbf{62.24} &61.6 \\ 
\cline{2-8}
& \multirow{BERT + AT + Mixup} & 90.85 & 90.87 & \textbf{87.30} & 86.83 &  59.66 &62.5\\ 
\cline{2-8}
& \multirow{BERT + TextFlint} & 89.71 & 88.18 &60.32  & 56.64 & 64.29 & 65.88\\
\hline\cline{1-8}
\textbf{50\%} & \multirow{BERT + AT} & 90.85 &91.11 & 87.50  & 90.41 & 59.17 &62.18 \\ 
\cline{2-8}
& \multirow{BERT + AT + Dropout} & 90.19 & 90.2 & \textbf{88.88} & 85.8 & \textbf{63.29} &60.83 \\ 
\cline{2-8}
& \multirow{BERT + AT + Mixup} &\textbf{90.92} & 89.76 & 88.00 &88.32 & 60.09 &\textbf{63.86} \\ 
\cline{2-8}
& \multirow{BERT + TextFlint} & 89.55 &89.05  & 53.49 &59.93  &62.72  &65.48 \\
\hline\cline{1-8}
\textbf{100\%} & \multirow{BERT + AT} & 90.52 & 90.82 &  87.74  &90.34  & 57.14 &57.76 \\ 
\cline{2-8}
& \multirow{BERT + AT + Dropout} &90.16  & 90.76 & 88.45 & 88.46 & \textbf{61.28} &60.25 \\ 
\cline{2-8}
& \multirow{BERT + AT + Mixup} & \textbf{90.53} &90.81  & \textbf{90.21}&  86.59 & 59.92 & 60.43\\ 
\cline{2-8}
& \multirow{BERT + TextFlint} &87.31  & 85.83 &59.12  & 60.43 & 63.47 & 69.05\\
\hline
\end{tabular}
\caption{F1 Scores on the Original CoNLL 2003 Test Set (ID) and its Challenging Set (CS); Expert-Guided Augmented Data for Training (AT)}
\label{tab:f1_main_results}
\end{table*}
